An empirical study of Conv-TasNet

Conv-TasNet is a recently proposed waveform-based deep neural network that achieves state-of-the-art performance in speech source separation. Its architecture consists of a learnable encoder/decoder and a separator that operates on top of this learned space. Various improvements have been proposed to Conv-TasNet. However, they mostly focus on the separator, leaving its encoder/decoder as a (shallow) linear operator. In this paper, we conduct an empirical study of Conv-TasNet and propose an enhancement to the encoder/decoder that is based on a (deep) non-linear variant of it. In addition, we experiment with the larger and more diverse LibriTTS dataset and investigate the generalization capabilities of the studied models when trained on a much larger dataset. We propose cross-dataset evaluation that includes assessing separations from the WSJ0-2mix, LibriTTS and VCTK databases. Our results show that enhancements to the encoder/decoder can improve average SI-SNR performance by more than 1 dB. Furthermore, we offer insights into the generalization capabilities of Conv-TasNet and the potential value of improvements to the encoder/decoder.

==> z_Notes.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Observationss:
Linear encoder&decoder reverts phase, deep keep protects it
In single speaker case, deep encoder&decoder results in better performance too, indicating a deeper understanding of the input waveform.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% E-mails:
\{bkadi,~mhorg,~jpons,~vzkuma\}@dolby.com
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% First abstract:

Speech separation methods have experienced steadfast success in difficult scenarios where prior information about the speakers is not available and the mixture has a single channel. Although many succesful methods have historically relied on time-frequency representations of the signal, recent works based on the Conv-TasNet architecture have showed the viability of performing the task of speech separation directly in the waveform domain. We argue that the learned yet linear transformation is the backbone of Conv-TasNet and we take another step to richer encodings by learning a nonlinear transformation. We show that this design choice leads to consistent performance improvement without losing the favorable properties of Conv-TasNet such as real time computation, small model size, short latency. Specifically, the proposed architecture, Conv-TasNet++ achieves \textcolor{red}{?} dB scale invariant signal to noise ratio improvement when compared to a Conv-TasNet architecture with more than twice the parameter count. When parameter counts are equal, this number increases up to \textcolor{red}{?} dB. Additionally, we utilize a novel methodology for testing the generalization properties of a speech separation network which enables a deeper understanding of the network's performance. All in all, this work encompasses ideas that take source separation and its performance evaluation to the next step.

Table~\ref{tab:5.1MSNR} shows results.

% \begin{table}[ht]
% \caption{Objective metrics for small model (5.1M parameters)}
% \label{tab:5.1MSNR}
% \begin{tabular}{|
% >{\columncolor[HTML]{C0C0C0}}c |cccccc}
% \hline
% {\color[HTML]{000000} E} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}{\color[HTML]{000000} N}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}{\color[HTML]{000000} H}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}{\color[HTML]{000000} SI-SNRi}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}{\color[HTML]{000000} Max SI-SNRi}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}{\color[HTML]{000000} Min SI-SNRi}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}{\color[HTML]{000000} SDRi}} \\ \hline
% 0 & 512 & 512 &  &  &  &  \\ \cline{1-1}
% 1 &  &  &  &  &  &  \\ \cline{1-1}
% 2 &  &  &  &  &  &  \\ \cline{1-1}
% 3 &  &  &  &  &  &  \\ \cline{1-1}
% 4 &  &  &  &  &  &  \\ \cline{1-1}
% 5 &  &  &  &  &  &  \\ \cline{1-1}
% \end{tabular}
% \end{table}

% Table~\ref{tab:12.8MSNR} shows some other results.

% \begin{table}[ht]
% \caption{Objective metrics for large model (12.8M parameters)}
% \label{tab:12.8MSNR}
% \begin{tabular}{|
% >{\columncolor[HTML]{C0C0C0}}c |cccccc}
% \hline
% {\color[HTML]{000000} E} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}{\color[HTML]{000000} N}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}{\color[HTML]{000000} H}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}{\color[HTML]{000000} SI-SNRi}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}{\color[HTML]{000000} Max SI-SNRi}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}{\color[HTML]{000000} Min SI-SNRi}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}{\color[HTML]{000000} SDRi}} \\ \hline
% 0 & 1024 & 1320 &  &  &  &  \\ \cline{1-1}
% 1 &  &  &  &  &  &  \\ \cline{1-1}
% 2 &  &  &  &  &  &  \\ \cline{1-1}
% 3 &  &  &  &  &  &  \\ \cline{1-1}
% 4 &  &  &  &  &  &  \\ \cline{1-1}
% 5 &  &  &  &  &  &  \\ \cline{1-1}
% \end{tabular}
% \end{table}

%Speech separation methods have experienced steadfast success in difficult scenarios where prior information about the speakers is not available and the mixture has a single channel. Although many succesful methods have historically relied on time-frequency representations of the signal, recent works based on the Conv-TasNet architecture have showed the viability of performing the task of speech separation directly in the waveform domain. In this work, we take a step back and evaluate (subjectively and objectively) different variants of this state-of-the-art model to gain insights on what's importaaaaaaaant (STILL NEED TO WORK OUT THE ABSTRACT, DEPENDING ON OUR ACTUAL CONTRIBUTIONS!)
% IDEAS: % that a learned linear transformation that is optimized for the task of speech separation is also a viable alternative. contrast linear with deep.
% FURTHER IDEAS FOR THE ABSTRACT: % We argue that the learned yet linear transformation is the backbone of Conv-TasNet and we take another step to richer encodings by learning a nonlinear transformation. We show that this design choice leads to consistent performance improvement without losing the favorable properties of Conv-TasNet such as real time computation, small model size, short latency. Specifically, the proposed architecture, Conv-TasNet++ achieves \textcolor{red}{?} dB scale invariant signal to noise ratio improvement when compared to a Conv-TasNet architecture with more than twice the parameter count. When parameter counts are equal, this number increases up to \textcolor{red}{?} dB. Additionally, we utilize a novel methodology for testing the generalization properties of a speech separation network which enables a deeper understanding of the network's performance. All in all, this work encompasses ideas that take source separation and its performance evaluation to the next step.

%%$x$ is partitioned into segments of $L$ consecutive samples with stride $S$. Segments $ x_k \in \mathbb{R}^L,~k \in \big[ K \big]$ are used as the input units to be separated. Notice that due to stride, $K = \frac{T - L}{S} + 1$. Formally $x_k = \text {vec} \bigg(\Big\{x_t \Big\}_{t=(k-1)S+1}^{(k-1)S+L} \bigg)$, where the vec$(\cdot)$ operator vectorizes a set of samples.

